LookingGlass: Generative Anamorphoses via Laplacian Pyramid Warping

Anamorphosis refers to a category of images that are intentionally distorted, making them unrecognizable when viewed directly. Their true form only reveals itself when seen from a specific viewpoint, which can be through some catadioptric device like a mirror or a lens. While the construction of these mathematical devices can be traced back to as early as the 17th century, they are only interpretable when viewed from a specific vantage point and tend to lose meaning when seen normally. In this paper, we revisit these famous optical illusions with a generative twist. With the help of latent rectified flow models, we propose a method to create anamorphic images that still retain a valid interpretation when viewed directly. To this end, we introduce Laplacian Pyramid Warping, a frequency-aware image warping technique key to generating high-quality visuals. Our work extends Visual Anagrams (arXiv:2311.17919) to latent space models and to a wider range of spatial transforms, enabling the creation of novel generative perceptual illusions.

==> figtex-teaser.tex <==
\begin{figure*}[t!]
  \centering
   \includegraphics[width=1.0\linewidth]{images-teaser.pdf}

   \caption{We propose a method to generate ambiguous anamorphosis, \ie images that reveals another image when viewed from some catadioptric devices such as a conic or cylindrical mirror.}
   \label{fig:teaser}
\end{figure*}

